Irregularity of distribution in Wasserstein distance

We study the non-uniformity of probability measures on the interval and the circle. On the interval, we identify the Wasserstein-$p$ distance with the classical $L^p$-discrepancy. We thereby derive sharp estimates in Wasserstein distances for the irregularity of distribution of sequences on the interval and the circle. Furthermore, we prove an $L^p$-adapted Erd\H{o}s$-$Tur\'{a}n inequality.

==> colemacros.tex <==
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Ham}{\mathbb{H}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eps}{\varepsilon}
\newcommand{\al}{\alpha}
\newcommand{\Om}{\Omega}
\newcommand{\bd}{\partial}
\newcommand{\h}[1]{\hat{#1}}
\newcommand{\s}[1]{\mathscr{#1}}
\newcommand{\m}[1]{\mathcal{#1}}
\newcommand{\f}[1]{\mathfrak{#1}}
\newcommand{\dn}{\mathrm{d}}
\newcommand{\ds}{\,\mathrm{d}}
\renewcommand{\d}{\;\mathrm{d}}
\newcommand{\Der}{\mathrm{D}}
\newcommand{\del}{\nabla}
\newcommand{\der}[2]{\frac{\dn #1}{\dn #2}}
\newcommand{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\abs}[1]{\left |#1 \right|}
\newcommand{\norm}[1]{\left \|#1 \right\|}
\newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\ti}[1]{\tilde{#1}}
\newcommand{\ubar}[1]{\underline{#1}}
\newcommand{\tbf}[1]{\textup{\textbf{#1}}}
\newcommand{\trm}[1]{\textup{\textrm{#1}}}
\newcommand{\id}[1]{\op{id}_{#1}}
\newcommand{\anon}{\,\cdot\,}
\renewcommand{\Re}{\op{Re}}
\renewcommand{\Im}{\op{Im}}
\newcommand{\Ker}{\op{ker}}
\newcommand{\Image}{\op{im}}
\newcommand{\Span}{\op{span}}
\newcommand{\supp}{\op{supp}}
\newcommand{\trans}[1]{\tensor*[^t]{#1}{}}
\newcommand{\smooth}[1]{\m{C}_c^\infty(#1)}
\newcommand{\arccot}{\op{arccot}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\noorm}[1]{\left|\left \|#1 \right\|\right|}
\newcommand{\MLoc}{\m M_{c,\text{loc}}}
\newcommand{\BM}{Brownian motion~}
\renewcommand{\And}{\quad \textrm{and} \quad}
\newcommand{\For}{\quad \textrm{for }}
\newcommand{\ForAll}{\quad \textrm{for all }}
\newcommand{\nab}{\nabla}
\newcommand{\trdeg}{\op{tr\,deg}}
\newcommand{\gr}{\op{gr}}
\newcommand{\rees}{\op{Rees}}
\newcommand{\Spec}{\op{Spec}}
\renewcommand{\hom}[2]{\op{Hom}(#1, #2)}
\renewcommand{\div}{\op{div}}
\newcommand{\bbraket}[1]{\left \langle \! \left \langle #1 \right \rangle \! \right \rangle}
\newcommand{\power}[1]{{#1}[\![X]\!]}
\newcommand{\laurent}[1]{{#1}(\!(X)\!)}
\DeclareMathOperator*{\Dlim}{D-lim}
\DeclareMathOperator*{\Clim}{C-lim}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\mr}{\mathring}
\newcommand\smallO{
  \mathchoice
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}% \displaystyle
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}% \textstyle
    {\scalebox{.9}{$\scriptscriptstyle\mathcal{O}$}}% \scriptstyle
    {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
  }

\newcommand{\nakedi}{\mathrm{i}}
\let\temp\i
\let\i\nakedi
\let\nakedi\temp
\let\temp\undefined

\newcommand{\smallbar}[1]{\overline{#1}}
\let\temp\bar
\let\bar\smallbar
\let\smallbar\temp
\let\temp\undefined
